SSN: Soft Shadow Network for Image Compositing

We introduce an interactive Soft Shadow Network (SSN) to generates controllable soft shadows for image compositing. SSN takes a 2D object mask as input and thus is agnostic to image types such as painting and vector art. An environment light map is used to control the shadow's characteristics, such as angle and softness. SSN employs an Ambient Occlusion Prediction module to predict an intermediate ambient occlusion map, which can be further refined by the user to provides geometric cues to modulate the shadow generation. To train our model, we design an efficient pipeline to produce diverse soft shadow training data using 3D object models. In addition, we propose an inverse shadow map representation to improve model training. We demonstrate that our model produces realistic soft shadows in real-time. Our user studies show that the generated shadows are often indistinguishable from shadows calculated by a physics-based renderer and users can easily use SSN through an interactive application to generate specific shadow effects in minutes.

==> src/2_related_work_-_SIGG.tex <==
\section{Related Work}
We relate our work to soft shadow generation and image composition. Shadow synthesis is one of the oldest topics in computer graphics and we refer the reader to the state of the art report~\cite{woo1990survey} as well to the recent book~\cite{eisemann2016real}. We limit the review to soft shadow generation~\cite{soft-survey} and to the recent algorithm for image composition, relighting, and manipulation. 

\noindent\textbf{Soft Shadows:} One common method for soft shadow generation from a single area light source is its approximation by summing multiple hard shadows, and the common algorithms build on the seminal hard-shadow map generation~\cite{Crow77}. For example, the work~\cite{assarsson2003geometry} uses volumetric shadows that exploit object silhouettes of the shadow caster. So-called silhouette maps~\cite{shadowSil} also use the object silhouette to augment the information in shadow map for faster hard shadow computation, and they were also used for texture magnification~\cite{sen2004silhouette}. Many of the single light source estimations are aimed at real-time performance and they sacrifice the precision for speed of soft shadows calculation~\cite{brabec2002single,EGWR:EGWR03:208-218}. Contrary to silhouette-based approaches requiring full 3D object geometry, our algorithm estimates soft shadow from only a 2D binary mask of the object using deep learning. 

% Our algorithm also aims at the fast generation, but instead of sampling the input geometry, it estimates the soft shadow from the input binary mask and the image-based light.

Agrawala et al.~\cite{agrawala2000efficient} introduced two algorithms: layered attenuation maps that are precomputed, and coherence-based raytracing that uses the maps for soft shadows generation. Guennebaud et al.~\cite{guennebaud2006real} used projection of the object geometry back to the area light to estimate the coverage. This method uses a single shadow map to approximate soft shadows, and it also suffers from soft shadow overestimation. This drawback has been eliminated by~\cite{schwarz2007bitmask,HQASSM} that uses multi-resolution sampling. 

A class of algorithms generates soft shadows by image filtering that can be expressed as a convolution~\cite{soler1998fast}. The variance~\cite{donnelly2006variance} and convolution~\cite{annen2007convolution} shadow maps are methods that sample the shadow in linear time. Most of the methods that use precomputed soft shadows are unable to handle dynamic scenes and this drawback has been addressed by the method of~\cite{Annen08}. Our method uses an arbitrary image light map instead of a single light source and is also suitable for dynamically changing scenes with varying light conditions that can be modeled interactively. 

Global illumination algorithms provide soft shadows implicitly. Spherical harmonics~\cite{cabral1987bidirectional, sillion1991global, westin1992predicting} based methods render global illumination effects including soft shadows in real-time by precomputing coefficients in spherical harmonics bases, which is similar to our shadow bases. But each of our shadow bases can be computed in real-time while each spherical harmonics base involves expensive monte-carlo integration. Close to our method for fast soft shadow calculation during the training are point-sampling approaches used in importance sampling~\cite{Agarwal03,Ostromoukhov04}. We trade-off shadow accuracy for efficient model training.

\noindent\textbf{Image Relighting and shadow Synthesis: }
Our method belongs to the category of deep generative models~\cite{goodfellow2014generative, kingma2013auto} which can perform image synthesis and manipulation via semantic control~\cite{10.1145/3306346.3323023, brock2018large, odena2017conditional} or user guidance such as sketches and painting~\cite{isola2017image,park2019semantic}. 

Among them, deep image harmonization and relighting methods~\cite{shu2017portrait,sun2019single,tsai2017deep,Zheng_2020_CVPR} learn to adapt the subject's appearance to match the target lighting space. 
This line of works focuses mainly on the harmonization of the subject's appearance such as color, texture, or lighting style~\cite{sun2019single,sunkavalli2010multi,tao2010error}. 

% Soft shadow synthesis for 2D image compositing has been understudied. 

Shadow generation and harmonization can be achieved by estimating the environment lighting and the scene geometry from multiple views~\cite{10.1145/3306346.3323013}.
Given a single image, Hold-Geoffroy et al.~\cite{hold2017deep} and Gardner et al.~\cite{gardner2017learning} proposed methods to estimate lighting maps for 3D object compositing. However, neither the multi-view information nor the object 3D models are available in general 2D image compositing. Potentially, 3D reconstruction methods from a single image~\cite{fan2017point,hassner2006example,saito2019pifu} can close this gap, but they typically require a complex model architecture design for 3D representation and may not be suitable for time-critical applications such as interactive image editing. Also, the over simplified camera model in these methods often brings artifacts in the touching area between the occluder and the shadow receiver. More details will be discussed in ~\ref{fig:comparison_pifuhd}. Recent works ~\cite{liu2020arshadowgan, hu2019mask} explored rendering hard shadows using GAN based method. But those works cannot render soft shadows and lack shadow controls during image editing.

Our work aims to provide a highly controllable method, including manipulating shadow direction, softness, intensity, etc, for realistic soft shadow generation, which is an essential element for a convincing composite photo. Our method is trained to implicitly infer object 3D information from a 2D cutout mask regardless of their appearance and thus can be applied in general image compositing tasks for different image types.



